Safe Non-Stochastic Control of Control-Affine Systems: An Online Convex Optimization Approach

We study how to safely control nonlinear control-affine systems that are corrupted with bounded non-stochastic noise, i.e., noise that is unknown a priori and that is not necessarily governed by a stochastic model. We focus on safety constraints that take the form of time-varying convex constraints such as collision-avoidance and control-effort constraints. We provide an algorithm with bounded dynamic regret, i.e., bounded suboptimality against an optimal clairvoyant controller that knows the realization of the noise a prior. We are motivated by the future of autonomy where robots will autonomously perform complex tasks despite real-world unpredictable disturbances such as wind gusts. To develop the algorithm, we capture our problem as a sequential game between a controller and an adversary, where the controller plays first, choosing the control input, whereas the adversary plays second, choosing the noise's realization. The controller aims to minimize its cumulative tracking error despite being unable to know the noise's realization a prior. We validate our algorithm in simulated scenarios of (i) an inverted pendulum aiming to stay upright, and (ii) a quadrotor aiming to fly to a goal location through an unknown cluttered environment.

==> 6-Control.tex <==
\section{Application to Safe Non-Stochastic Control}\label{sec:control}

We apply \SafeOGD and \SafeAder to the online non-stochastic control problem \citep{agarwal2019online} with safety constraints, and present the first online controllers with safety guarantee and with bounded dynamic regret against any linear time-varying feedback control policy (\Cref{alg:SafeOGD_Control,alg:SafeAder_Control}, and \Cref{theorem:SafeOGD_Control,theorem:SafeAder_Control}, respectively). 

\subsection{The Safe Non-Stochastic Control Problem}\label{subsec:control_formulation}
To formulate the problem of \textit{Safe Non-Stochastic Control} (\Cref{prob:SafeNSC}), we first establish  notation and assumptions.

\myParagraph{Linear Time-Varying System}
We consider Linear Time-Varying (LTV) systems of the form
\begin{equation}
	x_{t+1} = A_{t} x_{t} + B_{t} u_{t} + w_{t}, \quad t=1, \ldots, T,
	\label{eq:LTV}
\end{equation}
where $x_t \in\mathbb{R}^{d_x}$ is the state of the system, $u_t \in\mathbb{R}^{d_u}$ is the control input, and $w_t\in\mathbb{R}^{d_x}$ is the process noise.  The system and input matrices, \ie $A_t$ and $B_t$, are known.


\begin{assumption}[Convex and Bounded Loss Function with Bounded Gradient]\label{assumption:cost}
The loss function $c_{t}(x_{t+1},u_t): \mathbb{R}^{d_{x}} \times \mathbb{R}^{d_{u}} \mapsto \mathbb{R}$ is convex in $x_{t+1}$ and $u_t$. Further, when $\|x\|\;\leq D_c$, $\|u\|\;\leq D_c$ for some $D_c>0$, then $\left|c_{t}(x, u)\right| \leq$ $\beta D_c^{2}$ and $\left\|\nabla_{x} c_{t}(x, u)\right\|\leq G_{c} D_c,\left\|\nabla_{u} c_{t}(x, u)\right\| \leq G_{c} D_c$, for given positive numbers $\beta$ and $G_c$.
\end{assumption} 

\begin{assumption}[Bounded System Matrices and Noise]\label{assumption:bounded_system_noise}
The system matrices and noise are bounded, \ie $\|A_t\|\; \leq \kappa_{A}$, $\|B_t\|\; \leq \kappa_{B}$, and $w_t \in \calW \triangleq \{w \mid \left\|w\right\| \leq W\}$ where $\kappa_{A}$, $\kappa_{B}$, and $W$ are given positive numbers.
\end{assumption}

Per \Cref{assumption:bounded_system_noise}, we assume no stochastic model for the process noise $w_t$: the noise may even be adversarial, subject to the bounds prescribed by $W$.

\myParagraph{Safety Constraints} We consider the states and control inputs for all $t$ must satisfy polytopic constraints of the form
\begin{equation}
    \begin{aligned}
        & x_t \in \calS_t \triangleq \{x \mid L_{x,t} x \leq l_{x,t}\}, \ \forall \{{w}_{\tau} \in \calW\}_{\tau=1}^{t-1}, \\
        & u_t \in \calU_t \triangleq \{u \mid L_{u,t} u \leq l_{u,t}\}, 
    \end{aligned}
    \label{eq:safety_constraints}
\end{equation}
for given $L_{x,t}$, $l_{x,t}$, $L_{u,t}$, and $l_{u,t}$.\footnote{Our results hold true also for any convex state and control input constraints. We focus in \cref{eq:safety_constraints} on only polytopic constraints for simplicity in the presentation.}

\myParagraph{Linear-Feedback Control Policy} We consider the linear state feedback control policy $u_{t} = K_{t} x_{t}$, where
\begin{equation}
    % K_{t} \in \calK_t \triangleq \{K \mid \| K \| \leq \kappa, \   \| A_t - B_t K\| \leq 1-\gamma \},
     \| K_t \|\; \leq \kappa, \   \| A_t - B_t K_t\|\; \leq 1-\gamma,
    \label{eq:Kt}
\end{equation}
for given $\kappa > 0$ and $\gamma \in (0,1)$, and $K_t$ is the control gain to be designed. The constraint of $\| K_t \|\; \leq \kappa$ ensures $K_t$ is chosen from a compact decision set, and the constraint of $\| A_t - B_t K_t\|\; \leq 1-\gamma$ ensures the closed-loop stability.

% At each time step $t$, the controller first chooses a control input $u_t \in \calU_t$ that ensures the system evolves to a safe state $x_{t+1} \in \calS_{t+1}$, then the system suffers a loss $c_t(x_{t+1},u_t)$. The noise $w_t$ and the loss function $c_t$ are revealed to the controller only after the control input $u_t$ is chosen.

\myParagraph{Problem Definition} We formally define the problem of \textit{Safe Non-Stochastic Control}:
\begin{problem}[Safe Non-Stochastic Control (\SafeNSC)]\label{prob:SafeNSC}
Assume the initial state of the system is safe, \ie $x_0 \in \calS_{0}$. At each $t=1,\ldots, T$, first a control input $u_t \in \calU_t$ is chosen; then, a loss function $c_t : \mathbb{R}^{d_{x}} \times \mathbb{R}^{d_{u}} \mapsto \mathbb{R}$ is revealed and the system evolves to state $x_{t+1} \in \calS_{t+1}$ and suffers a loss $c_t(x_{t+1},u_t)$. The goal is to guarantee states and control inputs that satisfy the constraints in \cref{eq:safety_constraints} for all $t$ and that minimize the dynamic policy regret defined below.
\end{problem}

\begin{definition}[Dynamic Policy Regret]\label{def:DyReg_control}
The \emph{dynamic policy regret} is defined as
\begin{equation}
	\DyRegNSC = \sum_{t=1}^{T} c_{t}\left(x_{t+1}, u_{t}\right)-\sum_{t=1}^{T} c_{t}\left(x_{t+1}^{*}, u_{t}^{*}\right),
	\label{eq:DyReg_control}
\end{equation}
where (i) both sums in \cref{eq:DyReg_control} are evaluated with the same noise $\{w_1,\ldots, w_T\}$,  which is the noise experienced by the system during its evolution per the control input $\{u_1,\ldots, u_T\}$, (ii) $u_{t}^{*} = -K_t^{*} x_{t}^{*}$ is the optimal linear feedback control input in hindsight, {\ie the optimal input given a priori knowledge of $c_t$ and of the realized noise $w_t$}, (iii) $x_{t}^{*}$ is the state reached by applying the sequence of optimal control inputs $\{u_{1}^{*}, \dots, u_{t-1}^{*}\}$, and (iv) $x_{t}^{*}$ and $u_{t}^{*}$ satisfy constraints defined in \cref{eq:safety_constraints} for all $t$.
\end{definition}



% \subsection{\SafeOGD and \SafeAder Algorithms for \SafeNSC}\label{subsec:control_alg}
% We present \SafeOGD and \SafeAder's application to the problem of \SafeNSC (\Cref{prob:SafeNSC}). 

\input{Alg/Alg-SafeOGD-Control.tex}
\input{Alg/Alg-SafeAder-Control.tex}



\subsection{\SafeOGD Algorithm for \SafeNSC}\label{subsec:SafeOGD_control}
We present \SafeOGD for \SafeNSC in \Cref{alg:SafeOGD_Control}. The algorithm first initializes $K_1 \in \calK_1$ (line 1). At each iteration $t$, \Cref{alg:SafeOGD_Control} evolves to state $x_{t+1}$ with the control inputs $u_t = -K_t x_t$ and obtain the noise $w_t$ (lines 3-4). After that, the cost function is revealed and the algorithm suffers a loss of $c_t(x_{t+1},u_t)$ (line 4). Then \Cref{alg:SafeOGD_Control} expresses $c_t(x_{t+1},u_t)$ as a function of $K_t$, denoted as $f_t(K_t) \triangleq c_t((A_t - B_t K_t) x_t + w_t, - K_t x_t)$ ---which is convex in $K_t$, given $A_t$, $B_t$, $x_t$, and $w_t$, per \Cref{lemma:cvx_K} below--- and obtains the gradient $\nabla_K f_t(K_t)$ (lines 6-7). To ensure safety, \Cref{alg:SafeOGD_Control} constructs the domain set $\calK_{t+1}$ per \Cref{lemma:calK_t} (line 8). Finally, \Cref{alg:SafeOGD_Control} updates the control gain and projects it back to the domain set $\calK_{t+1}$ (lines 9-10).


\begin{lemma}[Convexity of Loss function in Control Gain]\label{lemma:cvx_K}
The loss function $c_{t}\left(x_{t+1}, u_{t}\right) : \mathbb{R}^{d_x} \times \mathbb{R}^{d_u} \blue{\rightarrow} \mathbb{R}$ is convex in the control gain $K_t$.
\end{lemma}


\begin{lemma}[Construction of Time-Varying Domain Set with Safety Guarantee]\label{lemma:calK_t}
By choosing $K_t \in \calK_t$, where
\begin{equation}
    \begin{aligned}
    \calK_t &\triangleq \{  K \mid - L_{x,t} B_t K x_t  \leq l_{x,t} - L_{x,t} A_t x_t - W\|L_{x,t}\|, \\
     & -L_{u,t} K x_t \leq l_{u,t}, \  \| K \|\; \leq \kappa, \   \| A_t - B_t K\| \;\leq 1-\gamma \},
    \end{aligned}
    \label{eq:lemma_calK_t}
\end{equation}
we guarantee $x_{t+1} \in \calS_{t+1}$ and $u_t \in \calU_t$ at each time step $t$.
\end{lemma}

\subsection{\SafeAder for \SafeNSC}\label{subsec:SafeAder_control}
We present \SafeAder for \SafeNSC in \Cref{alg:SafeAder_Control}. 
Particularly, \Cref{alg:SafeAder_Control} initializes the number of base-learners, their corresponding step sizes, and their initial weights, per the following equations:
\begin{align}
    &N=\left\lceil\frac{1}{2} \log _2(1+\frac{8T}{7})\right\rceil+1 = \mathcal{O}(\log T), \label{eq:SafeAder_N_control} \\
    &\mathcal{H}=\left\{\eta_i \mid \eta_i=2^{i-1} \sqrt{\frac{7 D_f^2}{2 T G_f^2}}, i \in \{1, \dots, N\}\right\},	\label{eq:SafeAder_step_size_pool_control} \\
    &p_{1, i}=\frac{1}{i(i+1)} \cdot \frac{N+1}{N}, \text{ for any } i \in \{1, \dots, N\},\label{eq:SafeAder_initial_weight_control}
\end{align}

The algorithm also sets the step size of meta-learner as
\begin{equation}
	\epsilon=\sqrt{2 / (T D_f^2 G_f^2)}
	\label{eq:SafeAder_meta_step_size_control}
\end{equation}
with $G_f$ and $D_f$ defined as in \Cref{lemma:Gradient} and \Cref{lemma:K_norm}.

At each iteration $t$, \Cref{alg:SafeAder_Control} receives $K_{t,i}$ from all base-learners (line 3). Then, \Cref{alg:SafeAder_Control} calculates $K_t = \sum_{i=1}^{N}p_{t,i} K_{t,i}$ and outputs the control inputs $u_t = -K_t x_t$ (lines 4-5). Afterwards, the noise $w_t$ is calculated when $x_{t+1}$ is observed (line 6). Then, the cost function is revealed and the algorithm suffers a loss of $c_t(x_{t+1},u_t)$ (line 7). Next, \Cref{alg:SafeAder_Control} expresses the loss function as a function of $K_t$, and obtains the gradient (lines 8-9). Finally, the meta-learner and base-learners update the weights $\boldsymbol{p}_{t+1}$ and $K_{t+1,i}$ for the next iteration (lines 10-15). 

% The initialization of \Cref{alg:Meta_OFW_Control} is detailed as below.
% \myParagraph{Step size pool} We initiate 
% \begin{equation}
% 	N=\left\lceil\frac{1}{2} \log_2(\frac{2\beta D^2 T + k_5}{k_3})\right\rceil+1 = \mathcal{O}(\log T)
% 	\label{eq:base_learners_N_control}
% \end{equation} 
% base-learners, with step size pool set as
% \begin{equation}
% 	\mathcal{H}=\left\{\eta_i \mid \eta_i=2^{i-1} \sqrt{\frac{k_3}{T D_f}} \leq 1, i \in \{1, \dots, N\}\right\},
% 	\label{eq:step_size_pool_control}
% \end{equation}
% where $k_3 = 2\sqrt{2}\beta D^2$, $k_5 = k_3 + 2\beta D^2$, and $D$, $D_f$ are defined in \Cref{lemma:loss_Mspace_property}.

% \myParagraph{Initial weight}
% We initiate the weight $\boldsymbol{p}_{0} \in \Delta_{N}$ of each base-learner $\calB_i$ as
% \begin{equation}
% 	 p_{0, i}=\frac{1}{i(i+1)} \cdot \frac{N+1}{N}, \text{ for any } i \in \{1, \dots, N\}.
% 	 \label{eq:initial_weight_control}
% \end{equation}

% \myParagraph{Step size of meta-learner} 
% We set the step size of meta-learner as
% \begin{equation}
% 	\varepsilon=\sqrt{2 /\left((2 \lambda+G_f)(\lambda+G_f) D_f^2 T\right)},
% 	\label{eq:theorem_MetaOFW_meat_step_size_control}
% \end{equation}
% with $\lambda = (H+2)^2 L_f$, and $L_f$, $G_f$ defined in \Cref{lemma:loss_Mspace_property}.


\subsection{Dynamic Policy Regret Analysis}\label{subsec:control_regret}

We present dynamic policy regret bounds of \Cref{alg:SafeOGD_Control,alg:SafeAder_Control} against any sequence of linear feedback control policy in \Cref{theorem:SafeOGD_Control,theorem:SafeAder_Control}, respectively.

\begin{theorem}[Dynamic Policy Regret Bound of \Cref{alg:SafeOGD_Control}]\label{theorem:SafeOGD_Control}
Consider the \SafeNSC problem. \SafeOGD per \Cref{alg:SafeOGD_Control} with step size $\eta=\calO\left(\frac{1}{\sqrt{T}}\right)$ achieves against any linear feedback control policy $({K}^\star_1, \dots, {K}^\star_T) \in \calK_1 \times \cdots \times \calK_T$
% \begin{equation}
%     \DyRegNSC \leq \frac{\eta T G_f^2}{2} + \frac{7 D_f^2}{4 \eta} + \frac{D_f C_T}{\eta} + \frac{D_f S_T}{\eta}.
%     \label{eq:theorem_SafeOGD_bound_init}
% \end{equation}
% Choosing the step size $\eta=\calO\left(\frac{1}{\sqrt{T}}\right)$, we have 
\begin{equation}
    \DyRegNSC \leq \calO\left(\sqrt{T}\left(1+C_{T}+S_{T}\right)\right).
   	\label{eq:theorem_SafeOGD_control_bound}
\end{equation}
\end{theorem}

\begin{theorem}[Dynamic Policy Regret Bound of \Cref{alg:SafeAder_Control}]\label{theorem:SafeAder_Control}
Consider the \SafeNSC problem. \SafeAder per \Cref{alg:SafeAder_Control} achieves against any sequence of linear feedback control policy $({K}^\star_1, \dots, {K}^\star_T) \in \calK_1 \times \cdots \times \calK_T$ 
	\begin{equation}
		\begin{aligned}
			\DyRegNSC & \leq {\mathcal{O}}\left(\sqrt{ T\left(1+C_T+S_T\right)} \right).
		\end{aligned}
		\label{eq:theorem_MetaOFW_bound_control}
	\end{equation}	
\end{theorem}

% \begin{remark}[Closed-Loop Stability \cite{karapetyan2022implications,nonhoff2022relation}]
% \end{remark}

\begin{remark}[Novelty of \Cref{theorem:SafeOGD_Control,theorem:SafeAder_Control}]
\Cref{theorem:SafeOGD_Control} and \Cref{theorem:SafeAder_Control} guarantee dynamic regret bounds with safety guarantees against an optimal \emph{time-varying linear feedback policy} in hindsight, \ie against $\{K_t^*\}_{t=1,\dots,T}$. 
This is different than non-stochastic control algorithms that
(i) consider no safety guarantees \cite{agarwal2019online,gradu2020adaptive,simchowitz2020improper,zhang2022adversarial,zhao2022non}; 
(ii) compete against an optimal time-varying control policy with pre-specified stabilizing linear feedback policy \cite{zhao2022non}, or an optimal time-\underline{in}variant linear feedback policy over the entire horizon or any time interval \cite{agarwal2019online,li2021online,gradu2020adaptive,simchowitz2020improper,zhang2022adversarial}; and
(iii)  require a priori pre-stabilizing linear feedback policy as in all aforementioned literature.
\end{remark}









\subsection{Numerical Evaluations}\label{subsec:control_exp}
We compare \Cref{alg:SafeOGD_Control} and \Cref{alg:SafeAder_Control} with $H_2$ ana $H_\infty$ controllers \cite{hassibi1999indefinite} in simulated scenarios of safe control of linear time-invariant systems. Supplementary numerical experiments that compare \Cref{alg:SafeOGD_Control} and \Cref{alg:SafeAder_Control} with \OCOM controllers \citep{agarwal2019online,zhao2022non} are presented in Appendix~\ref{app:supp_exp}. 
% \blue{Our code will be open-sourced via a link here.} 


\input{Table/Table-SafeControl.tex}

\myParagraph{Simulation Setup} 
We consider the linear system 
\begin{equation}\label{eq:exp_sys}
    \begin{aligned}
        x_{t+1} &= a x_{t} + b u_{t} + w_{t},
    \end{aligned}
\end{equation}
    where $x_t, \; u_t \in \mathbb{R}$, $a=0.9$, $b=0.6$, ${w}_{t}$ subject to $\| w_t \|\; \leq 1$ is sampled from various distributions, \ie Gaussian, Uniform, Gamma, Beta, Exponential, and Weibull distributions. The state and control input constraints are $\| x_t \|\; \leq 2$ and $\| u_t \|\; \leq 2.5$ for all $t$. The loss function has the form $c_t(x_{t+1},u_t) =  x_{t+1}^2 + u_t^2$ for all $t$. We choose the total time horizon as $T=200$.
 


\myParagraph{Results} 
The results are summarized in \Cref{table_safety_exp}. The \SafeOGD- and \SafeAder-based controllers achieve lower cumulative costs than the $H_2$ and $H_\infty$ controllers among all tested noise distributions, except for the case of Gaussian noise where the $H_2$ controller is better, as expected since it is the optimal controller in the presence of Gaussian noise.  

\begin{remark}[\SafeOGD \vs~\SafeAder]
    The performance of \SafeOGD and \SafeAder controllers are close across all tested noise distributions. The \SafeOGD controller requires step size tuning to achieve such behaviors. By contrast, the \SafeAder controller needs no step size tuning, but it requires more computational time since it has multiple \SafeOGD as subroutines.
\end{remark}




==> preamble_packages.tex <==

%!TEX root = main.tex

% LC: debug
%==========================================================================
%\usepackage{refcheck}
%\usepackage[notref]{showkeys}
%==========================================================================

% LC: to be used for TRO
%==========================================================================
% \usepackage{mathptmx} % assumes new font selection scheme installed
%\usepackage{times} % assumes new font selection scheme installed
%==========================================================================
\usepackage{comment}
\usepackage{siunitx}
\usepackage{relsize}
\usepackage{ifthen}

\usepackage[caption=false]{subfig}

% \begin{comment}
% % Fancy formatting 
% \usepackage[tracking=false,kerning=true,spacing=true]{microtype}
% \usepackage[caption=false]{subfig}

% \usepackage[style=numeric-comp,sorting=none,firstinits=true, maxnames=3,bibstyle=numeric,abbreviate=false,defernums=true,eprint=false,backend=bibtex]{biblatex}
% \renewcommand{\bibfont}{\footnotesize}
% % \DeclareFieldFormat[article]{pages}{#1}%
% % \DeclareFieldFormat[inproceedings]{pages}{#1}%

% \AtEveryBibitem{%
%   \ifentrytype{article}{%
%     \clearfield{pages}%
%   }{%
%   }%
%   \ifentrytype{inproceedings}{%
%     \clearfield{pages}%
%   }{%
%   }%
% }
% \end{comment}

% \bibliography{commons/bib/strings_long}
% \bibliography{commons/bib/all_only_one_w_pages}
% \bibliography{../../references/references}

% \usepackage[noadjust]{cite}
%\usepackage[vlined,ruled,linesnumbered]{algcompatible}
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{rotating}
\usepackage{color}
\usepackage{enumerate}
\usepackage[T1]{fontenc}
\usepackage{psfrag}
\usepackage{epsfig} % for postscript graphics files
%\usepackage{subfigure}
% \usepackage{hyperref}
\usepackage{booktabs}
\usepackage{graphicx,url}
\usepackage{multirow}
\usepackage{array}
\usepackage{latexsym}
\usepackage{amsfonts}
% \usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{xstring}
%\usepackage[noend]{algorithmic}
\usepackage{multirow}
\usepackage{xcolor}
\usepackage{prettyref}
\usepackage{flexisym}
\usepackage{bigdelim}
\usepackage{breqn} % load this last
\usepackage{listings}
\let\labelindent\relax
\usepackage{enumitem}
\usepackage{xspace}
\usepackage{bm}
\graphicspath{{./figures/}}
\usepackage{tikz}
\usetikzlibrary{matrix,calc}
\usepackage{epstopdf}
\usepackage{tikz-cd}
\DeclareGraphicsExtensions{.eps}
\usepackage{threeparttable}


%\usepackage{amsthm} % math
\usepackage{lineno}


%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%    dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/tex-archive/macros/latex/contrib/oberdiek/
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.

% *** GRAPHICS RELATED PACKAGES ***
%
%\ifCLASSINFOpdf
  % \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
%\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
%\fi


\usepackage{mdwlist}
\let\stditemize\itemize
\let\endstditemize\enditemize
\let\itemize\undefined
\makecompactlist{itemize}{stditemize}

%\let\stdenumerate\enumerate
%\let\endstdenumerate\endenumerate
%\let\enumerate\undefined
%\makecompactlist{enumerate}{stdenumerate}
 

